A Graph-Based Approach for Category-Agnostic Pose Estimation

Traditional 2D pose estimation models are limited by their category-specific design, making them suitable only for predefined object categories. This restriction becomes particularly challenging when dealing with novel objects due to the lack of relevant training data. To address this limitation, category-agnostic pose estimation (CAPE) was introduced. CAPE aims to enable keypoint localization for arbitrary object categories using a few-shot single model, requiring minimal support images with annotated keypoints. We present a significant departure from conventional CAPE techniques, which treat keypoints as isolated entities, by treating the input pose data as a graph. We leverage the inherent geometrical relations between keypoints through a graph-based network to break symmetry, preserve structure, and better handle occlusions. We validate our approach on the MP-100 benchmark, a comprehensive dataset comprising over 20,000 images spanning over 100 categories. Our solution boosts performance by 0.98% under a 1-shot setting, achieving a new state-of-the-art for CAPE. Additionally, we enhance the dataset with skeleton annotations. Our code and data are publicly available.

==> Figures/4_attn_maps/attn_maps.tex <==
\begin{figure}
  \centering
     % \setlength{\tabcolsep}{1pt}

  \begin{tabular}{ccccc}
    \includegraphics[width=0.18\textwidth]{Figures/4_attn_maps/0/0_2.png} & 
    \includegraphics[width=0.18\textwidth]{Figures/4_attn_maps/0/6_0.png} &
    \includegraphics[width=0.18\textwidth]{Figures/4_attn_maps/0/6_2.png} &
    \includegraphics[width=0.18\textwidth]{Figures/4_attn_maps/0/6_4.png} &
    \includegraphics[width=0.18\textwidth]{Figures/4_attn_maps/0/6_7.png} \\
    (a) & (b) & (c) & (d) & (e) \\
    Support & Support & 1st Layer & Last Layer & Predicted\\
    Skeleton & Keypoint & Heatmap & Heatmap & Location\\

    \end{tabular}
  \caption{\textbf{Attention Map Visualization}. We illustrate the cross-attention within the decoder, specifically between $F'_s$ and $F_q$. (a) illustrates the support skeleton, and (b) visualizes the searched keypoint in the support image. (c) In the initial layer, attention is centered solely on the queried keypoints. (d) In contrast, the final layer expands attention to neighboring keypoints based on skeletal connectivity. (e) Our decoder adeptly utilizes structural cues to accurately position keypoints within the query image.
  }
  \label{fig:attn_map}
\end{figure}

==> sec/6_ack.tex <==
\section{Acknowledgments}
Part of this research was supported by the Weinstein Institute and ISF grant 2132/23.

==> sec/old_experiments.tex <==
\section{Experiments}
\input{Figures/4_qualitative/qualitative}
We use the MP-100 dataset~\cite{xu2022pose} as our training and evaluation dataset, comprising samples drawn from existing category-specific pose estimation datasets. The MP-100 dataset encompasses a vast collection of over 20,000 images, spanning 100 distinct categories, with varying keypoint numbers up to 68 across different categories.
To facilitate model training and evaluation, the samples are divided into five distinct splits. Notably, each split ensures that training, validation, and test categories are mutually exclusive, meaning that the categories used for evaluation remain unseen during the training process.
The dataset includes partial skeleton annotations in various formats, including differences in the indexing of keypoints (some start from zero while others from one). To standardize and enhance the dataset, we adopted a unified format with comprehensive skeleton definitions for all categories. This process involved cross-referencing the original datasets and, where necessary, conducting manual annotations to ensure completeness and consistency.

To quantify our model's performance, we employ the Probability of Correct Keypoint (PCK) metric~\cite{yang2012articulated}, with a PCK threshold set at 0.2, following the conventions established by POMNet~\cite{xu2022pose}.

We show a qualitative comparison between our method and previous CAPE methods CapeFormer~\cite{Shi_2023_CVPR} and POMNet~\cite{xu2022pose} in Figure~\ref{fig:qualitative}. As can be seen, the structure information serves as a strong prior for localizing keypoints, helping in breaking symmetry and creating structure consistency between the keypoints.

\subsection{Implementation Details}
For a fair comparison, network parameters, training parameters, and data augmentations and pre-processing are kept the same as CapeFormer~\cite{Shi_2023_CVPR}:
Both the encoder and decoder have three layers and $\lambda_{heatmap}$ is set to $2.0$. 
The model is built upon MMPose framework~\cite{mmpose2020}, trained using Adam optimizer for 200 epochs with a batch size of 16, the learning rate is $10^{-5}$, and decays by 10× on the 160th and 180th epoch.

\subsection{Benchmark Results}
\input{tables/mp100}

We compare our method with the previous CAPE methods CapeFormer~\cite{Shi_2023_CVPR} and POMNet~\cite{xu2022pose} and three baselines: 
ProtoNet~\cite{snell2017prototypical}, MAML~\cite{finn2017model}, and Fine-tuned~\cite{nakamura2019revisiting}. Further details on the baseline models evaluation can be found in~\cite{xu2022pose}.

We report results on the MP-100 dataset under 1-shot and 5-shot settings in Table~\ref{Tab:mp100}. As can be seen, the enhanced baseline models, which are agnostic to the keypoints order, outperform previous methods and improve the average PCK by 0.94\% under the 1-shot setting and 1.60\% under the 5-shot setting.
Our graph-based method further improves performance, improving the enhanced baseline by 1.22\% under the 1-shot setting and 0.22\% under the 5-shot setting, achieving new state-of-the-art results for both settings.

We also show the scalability of our design. Similar to DETER-based models, employing a larger backbone improves performance. We show that our graph decoder design also enhances the performance of the larger enhanced baseline, improving results by 1.02\% and 0.34\% under 1-shot and 5-shot settings respectively.

% \subsection{Cross-Category Pose Estimation}
% \input{tables/cross_cat}
% To thoroughly assess our model's ability to generalize across vastly dissimilar categories, we follow~\cite{Shi_2023_CVPR} and evaluate our method under a cross-category setting.
% Within the MP-100 dataset, no category overlap exists between the training, validation, and test sets. Nevertheless, certain categories may exhibit similarities, such as different animal faces. Thus, we test our model on four general categories: human face, human body, vehicle, and furniture, and train it using the remaining categories.

% Results are shown in Table~\ref{Tab:cross_cat}. 
% As can be seen, we achieve state-of-the-art performance. The improvement in cross-category setting is more significant, which further demonstrates the generalization ability and robustness of the proposed method. 

\subsection{Ablation Study}
We conducted a number of ablation studies on the MP-100 dataset. We first evaluate our method using different backbones, showing the advantages of Swin Transformer architecture for localization tasks. 
We then show the contribution of the geometrical structure prior by evaluating our model using wrong skeleton relations.
We perform all experiments on the test set of MP-100 split1 under the 1-shot setting following~\cite{Shi_2023_CVPR, xu2022pose}.

\input{tables/backbones}
\paragraph{Different Backbones.} We assess our model's performance with various pre-trained backbones, including a CNN-based backbone (ResNet-50) and two distinct pre-trained transformer backbones, namely Dino~\cite{caron2021emerging, oquab2023dinov2} and Swin V2~\cite{liu2022swin}.
Dino and DinoV2 are self-supervised Vision Transformers trained via self-distillation, resulting in robust, finely detailed semantic features. Moreover, these encoded semantic representations are shared among related but distinct object categories.
Swin Transformer restructures self-attention with a window mechanism, balancing efficiency and performance for vision tasks. This hierarchical architecture has the flexibility to model at different scales and has linear computational complexity with respect to image size.

The results are summarized in Table~\ref{Tab:backbone}. It is evident that Swin-T outperforms other options, delivering superior results while maintaining efficiency comparable to the CNN-based backbone. In addition, using a larger backbone boosts performance, but at the price of efficiency and size.

\paragraph{The Contribution of Graph Structure.} To assess the contribution of the graph structure prior, we evaluate our method using random graph inputs by choosing edge connections randomly for each instance. This resulted in a performance decrease of 9.57\%, which validates the contribution of the graph decoder and the use of the structural information.

\input{Figures/4_attn_maps/attn_maps}

% \paragraph{Number of Decoder Layers.} We evaluate the impact of incorporating additional decoder layers into our architecture. Results are shown in Figure~\ref{fig:decoder_layers}. As can be seen, employing a larger number of decoder layers using our graph decoder shows better scalability, with boosted performance compared to the enhanced baseline for any number of decoder layers tested.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.45\textwidth]{Figures/4_num_decoders.pdf}
% 	\caption{\textbf{Number of Decoder Layers.}}
% 	\label{fig:decoder_layers}
% \end{figure}

\paragraph{Out-of-Distribution Performance.} To assess the robustness of our model, we evaluate it using images from different domains. Our model, which was trained on real images, demonstrates its adaptability and effectiveness across varying data sources such as cartoons and imaginary animals, created using a diffusion model. Results are shown in Figure ?.
\input{Figures/4_OOD/ood}

==> sec/old_method.tex <==
\section{Method}

\begin{figure*}
	\centering
	\includegraphics[width=0.95\textwidth]{Figures/3_arch.pdf}
	\caption{\textbf{Architecture Overview.} Our approach utilizes a pre-trained backbone to extract image features, followed by a transformer encoder that refines these features through self-attention. A similarity proposal generator is employed alongside a graph transformer decoder, enhancing keypoint localization accuracy with a focus on graph-oriented decoding.}
	\label{fig:intro}
\end{figure*}

Our method builds on top of CapeFormer~\cite{Shi_2023_CVPR}. For completeness, we describe it briefly below. Then, we describe an improved baseline that we establish by incorporating a few  adaptations into the architecture of CapeFormer following recent DETR advancements. Then, we show how we utilized the strong graph structure of the data in our architecture. Last, we introduce the supervision used to train our end-to-end model.

% Different Backbones
\subsection{The CapeFormer Model}
 Its design is similar to the DETR architecture and consists of 4 sub-networks:
\\
\begin{itemize}
\item \textbf{Shared backbone.} A pre-trained Resnet-50 is used to extract features from the input support and query images. 
To acquire the support keypoint features, we perform an element-wise multiplication between the support image feature map and keypoint masks. These masks are created by positioning Gaussian kernels centered at the support keypoints locations. In scenarios involving multiple support images, such as 5-shot settings, we calculate the average (in feature space) of the support keypoint features from different images.
This results in both the query feature map $\hat{F_q} \in \mathbb{R}^{hw \times C}$ and the support keypoint features $\hat{F_s} \in \mathbb{R}^{K \times C}$.
\item \textbf{Transformer encoder.} A transformer encoder is used to enhance the image features and facilitate the fusion of information between the support keypoint features and the query patch features. The encoder consists of three transformer blocks, each housing a self-attention layer. Before entering the self-attention layer, the input support keypoints and query features are concatenated and subsequently separated once more. The outputs are refined query feature map $F_q$ and refined support keypoint features $F_s$.

\item \textbf{Similarity-Aware Proposal Generator.} The proposal generator aligns support keypoint features with query features, resulting in similarity maps. From these maps, we select peaks to serve as the similarity-aware proposals. In pursuit of a balance between efficiency and versatility, a trainable inner-product mechanism is employed to explicitly model similarity.

\item \textbf{Transformer decoder.} To decode keypoint locations from the query feature map, a transformer decoder network is utilized. The Transformer decoder consists of three layers, with each layer including self-attention, cross-attention, and feed-forward blocks.
An iterative refinement strategy, inspired by prior work~\cite{cai2018cascade, teed2020raft, zhu2020deformable}, is applied to enable each decoder layer to predict coordinate deltas for the previous coordinate predictions. 
Additionally, similar to the approach in Conditional DETR~\cite{meng2021conditional}, the decoder utilizes the predicted coordinates to provide enhanced reference points for pooling features from the image feature map.
\\
\end{itemize}




\subsection{An Enhanced Baseline}


Following~\cite{lin2023detr}, our baseline model mostly tracks the original CapeFormer framework, experimenting with the following adaptations:
% except for the following adaptations:

\paragraph{Improved Backbone.} We use a stronger, transformer-based, SwinV2-T~\cite{liu2022swin} backbone, instead of the original ResNet-50~\cite{he2016deep} backbone, which can also provide a multi-scale feature map. After experimenting with various configurations, including scale fusion and single-scale feature maps, we found that applying a straightforward bilinear upsampling on the final feature layer yielded similar results while preserving simplicity. 
Additionally, we optimized the extraction of support keypoint features by employing a Gaussian kernel mask with lower variance, taking advantage of the enhanced feature quality from the new backbone. These simple adjustments led to a 3.2\% improvement in PCK.

% \paragraph{Iterative Refinement Stabilization} Following ~\cite{zhu2020deformable}, CapeFormer introduced a straightforward, yet efficient, iterative localization refinement mechanism to enhance detection performance. In this approach, each decoder layer iteratively improves localization predictions based on the information from the preceding layer. The iterative decoder blocks localization gradients back-propagation to stabilize training. 
% We found this method effective, yet not sufficient. In order to fully leverage to iterative scheme we found it necessary to block the gradient back-propagation of both the location prediction and the support feature refinement. This simple change resulted in an improvement of ?? PCK.

% % Look twice
\paragraph{Look Forward Twice.} We asses a look-forward twice scheme~\cite{zhang2022dino, jia2023detrs} to leverage the refined coordinates information derived from previous decoder layers. Although shown effective in detection tasks, we observed it did not improve performance for our keypoint localization task.

\paragraph{Disable Support Keypoint Identifier.} 

CapeFormer introduced a keypoint positional encoding, termed the "Support Keypoint Identifier". This encoding is generated via sinusoidal encoding of the keypoints' order.
However, while this encoding improves performance by a significant 3\% PCK, it introduces a dependency on the order of keypoints. Although the dataset contains diverse object categories, some of them share a common keypoint ordering. 

\shai{Maybe put this part in the Ablation. For now just state that we have to chosen to remove this encoding from our baseline.}

This became evident when we evaluated a model trained with this positional encoding on data of keypoints with reverse order. The result was a notable decrease of approximately 30\% in PCK, indicating that the model had become highly specialized for a specific keypoint format. This sharp decrease is not present when the positional encoding is not used.
We believe that category-agnostic pose estimation (CAPE) should not rely on such assumptions and should accommodate support keypoints without imposing a specific order. Therefore, we have chosen to remove this encoding from our baseline.

\subsection{Utilizing Graph Structure}
% The core idea of our work is that different keypoints have a geometrical structure that can be represented as a graph.

% The pose keypoints in the support images represent an undirected graph $G=(V, E)$. Each node $V=\{V_{i},i\in[1, N]\}$ corresponds to a skeleton with $N$ joints, and each edge $E$ represents a relation between two nodes. 

The core idea of our work is to take advantage of the geometrical structure encoded in the pose graph. To this end, the pose keypoints in the support images are represented by an undirected graph $G=(V, E)$, where $|V| = N$ and $E \subseteq V \times V$. $V_i$ denotes one of the $N$ joints and each edge $E_{ij}$ connects two nodes. 


\subsubsection{Skeleton Loss}
\shai{Consider moving to the ablation. We are not using this loss in practice.}

A na\"ive approach to utilizing the graph structure is to force features of the support and query image to be similar along an edge, which is defined by a straight line between 2 keypoints. We call this approach a skeleton loss. 
Denote the feature map of support and query images as $F_s$ and $F_q$ respectively. Given an edge $e \in E$, we sample the feature maps $k$ times along the edge from both feature maps to acquire $\{f_s^{e,i}, f_q^{e,i}\}, i \in [1, k]$. We then encourage the cosine similarity between $f_s^{e,i}$ and $f_q^{e,i}$ to be large:

\begin{equation}
L_{skeleton} = \sum_{e \in E} \sum_{i=1}^k (1-\frac{f_s^{e,i} \cdot f_q^{e,i}}{\lVert f_s^{e,i} \rVert \lVert f_q^{e,i} \rVert})
\end{equation}

This solution didn't improve performance. First, we had the strong assumption that the features along a straight line should be similar, which doesn't always hold. Second, this loss resulted in a smoother heatmap, as we only required the similarity of sampled features, while we should encourage distinct features to localize the keypoints.

Thus, we forced the cosine similarity between $f_s^i$ and $f_q^j$ to be large for $i=j$ and small for $i \neq j$. However, this constraint was too restrictive and resulted in worse performance.

\subsubsection{Graph Transformer Decoder}

\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{Figures/3_GraphDecoderV2.pdf}
	\caption{\textbf{Graph Transformer Decoder.} 
 \textbf{(a)} The decoder includes self-attention, cross-attention, and a feed-forward network. Self-attention encourages adaptive interactions among support keypoints, while cross-attention extracts localization information. \\
 \textbf{(b)} Previous feed-forward compromised of an MLP with 2 layers. \\
 \textbf{(c)} A novel feed-forward compromise of a GCN layer and subsequent linear layers enhances keypoint features and promotes information exchange among known connected keypoints.}
	\label{fig:graph_decoder}
\end{figure}

Another approach to leverage graph structure is to incorporate it into our model's architecture. We call this architecture Graph Transformer Decoder, utilizing a Graph Convolutional Network Layer (GCN) in the transformer layer, as can be seen in Figure~\ref{fig:graph_decoder}.

We recognize that self-attention, a mechanism that helps our model focus on relevant information, can be thought of as a graph convolutional network (GCN) with an learnable adjacency matrix. When we're dealing with pose estimation for a single category, this mechanism is sufficient for learning the relationships between keypoints and integrating a learned structure into the model.

However, for category-agnostic pose estimation (CAPE) tasks, where the model needs to work with various object categories, it's beneficial to explicitly consider the semantic connections between keypoints. This helps the model break symmetry, maintain consistent structure, and handle noisy keypoints by sharing information among neighboring keypoints.

The decoder is composed of three essential components: a self-attention block, a cross-attention block, and a feed-forward network.

Self-attention allows for the acquisition of adaptive interactions among the support keypoints. This mechanism ensures that each proposal possesses an understanding of the relative positions and attributes of other keypoints.
When dealing with an input keypoint feature $F_s^l$, we begin by passing it through a Multi-Head Self-Attention (MHSA) module, resulting in the transformed feature $F_s'$.

Subsequently, we use a cross-attention module, responsible for extracting relevant localization information from the query feature patches. This process enriches the representation of each support keypoint. Following a similar approach outlined in~\cite{Shi_2023_CVPR}, we enhance attentional focus on the proposed locations. This involves concatenating the keypoint localization embedding with the keypoint features, thereby promoting more precise localization. 
In this context, the localization embedding is the output of an MLP whose input is the predicted keypoint coordinates. The cross-attention inputs are $F_s'$ (concatenated with the localization embedding) as the queries, the patch features $F_q$ (concatenated with a positional encoding $P_q$) are the keys, and $F_q$ are the values, resulting in the transformed features $F_s''$.

Lastly, we employ a feed-forward network to process the output keypoint features. To incorporate prior geometrical knowledge, we introduce a graph neural network (GCN) layer. This GCN layer further concentrates the keypoint features, facilitating the exchange of information between known keypoint connections. To address the potential problem of excessive smoothing often observed in deep GCNs~\cite{li2018deeper, oono2019graph}, which can lead to a reduction in the distinctiveness of node characteristics and consequently a decline in performance, we introduce a linear layer for each node following the GCN layer.

The output value for an input $F_s'' \in \mathbb{R}^{C_{in} \times K}$ can be written as:
\begin{equation}
\widetilde{F_s''} =\sigma_{act} (W_{adj}F_s''\widetilde{A} + W_{self}F_s'')
\end{equation}
\begin{equation}
F_s^{l+1} = F_s'' + W_{linear}\widetilde{F_s''}
\end{equation}
Where $W_i \in \mathbb{R}^{C_{out} \times C_{in}}$ is a learnable parameter matrix, $\sigma_{act}$ is an activation function (ReLU), and $\widetilde{A}\in \mathbb{R}^{K \times K}$ is the symmetrically normalized form of the adjacency matrix $A \in [0,1]^{K \times K}$, which is defined as $a_{ij} = 1$ for node $v_j$ that is connected to node $v_i$ and $0$ elsewhere.

The output features $F_s^{l+1}$ are used to update the keypoints locations. We follow~\cite{Shi_2023_CVPR} and use the following update function:
\begin{equation}
 P^{l+1} = \sigma(\sigma^{-1}(P_l) + MLP (F_s^{l+1})) 
\end{equation}
where $\sigma$ and $\sigma^{-1}$ are the sigmoid and its inverse function.
The keypoints' positions from the last decoder layer are used as the final keypoints prediction.

\subsection{Training loss}
Following CapeFormer~\cite{Shi_2023_CVPR}, we use two supervision signals: a heatmap loss and an offset loss. The heatmap loss supervises the similarity metric and initial coordinates suggestion, while the offset loss supervises the localization output:
% Heatmap loss
\begin{equation}
\mathcal{L}_{heatmap} = \frac{1}{K \cdot H \cdot W}\sum_{i=1}^K \lVert \sigma(M_i)-H_i \rVert
\end{equation}
% L1 supervision for initial and refined positions
\begin{equation}
\mathcal{L}_{offset} = \frac{1}{L}\sum_{i=1}^L\sum_{i=1}^K |P_i^l - \hat{P_i}|
\end{equation}
where $M_i$ denotes the output similarity heatmap from the proposal generator, $\sigma$ is the sigmoid function, $H_i$ the ground-truth heatmap, $P_i$ the output location from the each layer and $ \hat{P_i}$ the ground-truth location.
The overall loss term is:
\begin{equation}
\mathcal{L} = \lambda_{heatmap} \cdot \mathcal{L}_{heatmap} + \mathcal{L}_{offset}
\end{equation}

==> supp_figs/mask/query_mask.tex <==
\begin{figure*}
\setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{1.5pt}
  \centering
  \begin{tabular}{c ccc}
     Support & GT & CapeFormer-T & \textbf{GraphCape} \\

    
    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/25_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_25_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_25_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/25_1.png}} \\


    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/30_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_30_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_30_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/30_1.png}} \\

    %     \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/38_0.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_38_1.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_38_1.png}} &
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/38_1.png}} \\

        \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/53_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_53_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_53_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/53_1.png}} \\

            \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/67_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_67_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_67_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/67_1.png}} \\
    
    %     \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/78_0.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_78_1.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_78_1.png}} &
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/78_1.png}} \\

    %     \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/79_0.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_79_1.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_79_1.png}} &
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/79_1.png}} \\

    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/82_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/gt_82_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/base_82_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/query/82_1.png}} \\

    \end{tabular}
  \caption{\textbf{Mask Query Results.} Qualitative results when masking the query image using the
enhanced baseline and our graph-based model. Although masking a large portion of the query image, using structure bias helps preserve structure consistency and break symmetry.
  }
  \label{fig:supp_mask_query}
\end{figure*}


==> supp_figs/mask/support_mask.tex <==
\begin{figure*}
\setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{1.5pt}
  \centering
  \begin{tabular}{c ccc}
     Support & GT & CapeFormer-T & \textbf{GraphCape} \\

    
    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/25_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/gt_25_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/base_25_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/25_1.png}} \\

    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/27_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/gt_27_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/base_27_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/27_1.png}} \\

    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/48_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/gt_48_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/base_48_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/48_1.png}} \\

    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/55_0.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/gt_55_1.png}} & 
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/base_55_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/55_1.png}} \\

    \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{Figures/mask/41_0.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{Figures/mask/gt_41_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{Figures/mask/41_1.png}} &
    \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{Figures/mask/44_1.png}} \\
    
    % \fcolorbox{purple}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/84_0.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/gt_84_1.png}} & 
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/base_84_1.png}} &
    % \fcolorbox{ForestGreen}{white}{\includegraphics[width=0.2\textwidth]{supp_figs/mask/support/84_1.png}} \\
    \end{tabular}
  \caption{\textbf{Mask Support Results.} Qualitative results when masking the support image using the
enhanced baseline and our graph-based model. Our model can predict keypoints even when a significant portion of the support image is masked, leveraging the power of graph structure.
  }
  \label{fig:supp_mask_supp}
\end{figure*}


==> tables/backbones.tex <==
\begin{table}
\centering
\caption{
\textbf{Pre-Trained Backbone Ablation.} PCK scores using different pre-trained backbones. Swin transformer combines superior results with efficient processing.
}
\small

\begin{tabular}{c|ccc}

\toprule
Backbone & \# Params[M] & FLOPS[G] & PCK$_{0.2}$ \\
\midrule
ResNet-50~\cite{he2016deep} & 25.5 & 4.1 & 87.71 \\
DinoV1-S~\cite{caron2021emerging} & 22.1 & 46.7 & 89.17 \\
DinoV2-S~\cite{oquab2023dinov2} & 22.1 & 46.7 &  90.34 \\
SwinV2-T~\cite{liu2022swin} & 28.3 & 4.4 & 91.19\\
SwinV2-S~\cite{liu2022swin} & 49.73 & 8.57 & 94.73\\

\bottomrule
\end{tabular}
\label{Tab:backbone}
\end{table} 

==> tables/cross_cat.tex <==
\begin{table}
\centering
\caption{
\textbf{Pre-Trained Backbone Ablation.} PCK scores using different pre-trained backbones. Swin transformer combines superior results with efficient processing.
}
\small
\begin{tabular}{c|cccc}

\toprule
Method & \begin{tabular}{@{}c@{}}Human \\ Body \end{tabular} & \begin{tabular}{@{}c@{}}Human \\ Face \end{tabular} & Vehicle & Furniture \\
\midrule
ProtoNet~\cite{snell2017prototypical} & 37.61 & 57.80 & 28.35 & 42.64 \\
MAML~\cite{finn2017model} & 51.93 & 25.72 & 17.68 & 20.09  \\
Fine-tuned~\cite{nakamura2019revisiting} & 52.11 & 25.53 & 17.46 & 20.76 \\
POMNet~\cite{xu2022pose} & 73.82 & 79.63 & 34.92 & 47.27  \\
CapeFormer~\cite{Shi_2023_CVPR} &  83.44 & 80.96 & 45.40 & 52.49  \\

Baseline-T &  X & X & X & X\\
\textbf{Ours-T} &  X & X & X & X \\
\midrule
Baseline-S &  X & X & X & X  \\
\textbf{Ours-S} &  X & X & X & X \\

\bottomrule
\end{tabular}

\label{Tab:cross_cat}
\end{table} 
